NPSim: Nighttime Photorealistic Simulation From Daytime Images With Monocular Inverse Rendering and Ray Tracing

Semantic segmentation is an important task for autonomous driving. A powerful autonomous driving system should be capable of handling images under all conditions, including nighttime. Generating accurate and diverse nighttime semantic segmentation datasets is crucial for enhancing the performance of computer vision algorithms in low-light conditions. In this thesis, we introduce a novel approach named NPSim, which enables the simulation of realistic nighttime images from real daytime counterparts with monocular inverse rendering and ray tracing. NPSim comprises two key components: mesh reconstruction and relighting. The mesh reconstruction component generates an accurate representation of the scene structure by combining geometric information extracted from the input RGB image and semantic information from its corresponding semantic labels. The relighting component integrates real-world nighttime light sources and material characteristics to simulate the complex interplay of light and object surfaces under low-light conditions. The scope of this thesis mainly focuses on the implementation and evaluation of the mesh reconstruction component. Through experiments, we demonstrate the effectiveness of the mesh reconstruction component in producing high-quality scene meshes and their generality across different autonomous driving datasets. We also propose a detailed experiment plan for evaluating the entire pipeline, including both quantitative metrics in training state-of-the-art supervised and unsupervised semantic segmentation approaches and human perceptual studies, aiming to indicate the capability of our approach to generate realistic nighttime images and the value of our dataset in steering future progress in the field.

==> ack.tex <==
%% ----------------------------------------------------------------------------
% BIWI SA/MA thesis template
%
% Created 09/29/2006 by Andreas Ess
% Extended 13/02/2009 by Jan Lesniak - jlesniak@vision.ee.ethz.ch
%% ----------------------------------------------------------------------------


\newpage

\chapter*{Acknowledgements}
First of all, I would like to express my deepest gratitude to my supervisor, Prof. Luc Van Gool and my advisor Dr. Christos Sakaridis, for their unwavering support, guidance, and encouragement throughout my thesis journey. Their expertise and passion for the subject have been instrumental in shaping my understanding of the field and inspiring me to pursue a career in research. Especially for my weekly meetings with Dr. Christos Sakaridis, his insightful feedback and countless discussions we had during our research endeavours. I'm truly fortunate to have had the opportunity to work in the Computer Vision Lab at ETH Zurich under his mentorship, and I'm immensely grateful for his patience and dedication in helping me grow as a researcher.

I would also like to extend my heartfelt thanks to my collaborators, who have been invaluable source of knowledge, kindness, and camaraderie. In particular, I would like to thank Konstantinos Tzevelekakis for his collaboration and kindness on this project, especially for his help during the data preparation and the model training. I am grateful to all members of the Computer Vision Lab for creating a stimulating and supportive environment, fostering a sense of community and enabling a fruitful exchange of ideas. Everyone who has helped me has contributed immensely to my personal and professional development.

Moreover, I'm also grateful to my home university, the University of Toronto, for giving me the chance to work as a researcher outside Canada and providing me with financial support, as well as to ETH Zurich, for accepting me as a research student and providing me with a strong world research environment.

Lastly, I would like to express my profound appreciation to my parents, and my entire family for their unconditional love, support, and encouragement. My friends for being a constant source of motivation, understanding and emotional support as I navigated through this period. My previous supervisors and collaborators, as their help and guidance have enabled my ability to better conduct scientific research. Their unwavering belief in me and my abilities has been the bedrock of my success, and their sacrifices have enabled me to reach my milestones again and again. I dedicate this thesis to everyone above, as s testament to their love and support.

==> text/discussion.tex <==
%% ----------------------------------------------------------------------------
% BIWI SA/MA thesis template
%
% Created 09/29/2006 by Andreas Ess
% Extended 13/02/2009 by Jan Lesniak - jlesniak@vision.ee.ethz.ch
%% ----------------------------------------------------------------------------
\newpage
\chapter{Discussion}
The discussion section gives an interpretation of what you have done \cite{day2006wap}:

\begin{itemize}
 \item \textit{What do your results mean?} Here you discuss, but you do not recapitulate results. Describe principles, relationships and generalizations shown. Also, mention inconsistencies or exceptions you found.
 \item \textit{How do your results relate to other's work?} Show how your work agrees or disagrees with other's work. Here you can rely on the information you presented in the ``related work'' section.
 \item \textit{What are implications and applications of your work?} State how your methods may be applied and what implications might be. 
\end{itemize}

\noindent Make sure that introduction/related work and the discussion section act as a pair, i.e. ``be sure the discussion section answers what the introduction section asked'' \cite{day2006wap}. 
% Pre
% Motivation
% Related work
% Technical details
% Results
% Conclusion
% 2/3 slides of munites, not over crowded, slides orientation

